Buildings for Synthesis with Clifford+R

We study the problem of exact synthesis for the Clifford+R gate set and give the explicit structure of the underlying Bruhat-Tits building for this group. In this process, we also give an alternative proof of the arithmetic nature of this gate set.

==> eptcsdata.tex <==
\providecommand{\firstpage}{144}
\providecommand{\publicationstatus}{J. van de Wetering, O. Oreshkov, and A.B. Sainz (Eds.):\\
Quantum Physics and Logic 2026 (QPL 2026)\\
EPTCS 456, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.456.5}{10.4204/EPTCS.456.5}}

